PRIME: Towards Verifiable Evidence-Grounded Reasoning in LLM Agents

LLM agents are used to check records against an organization's requirements, for example whether a vulnerability report is ready for investigation. Requirements often allow several ways to be met, such as a severity rating with a curator-reviewed advisory or a published advisory link. Agents fail by accepting a report after a required check has failed, or by settling for a weaker conclusion without trying another way that could still succeed. We introduce PRIME (Precommitted Rules for Inference from Minimal Evidence). Before checking, it fixes evidence routes specifying how each conclusion may be justified. A separate program records each check result and refuses any conclusion the results do not justify. It also points the agent to checks that could justify a stronger conclusion, or runs them itself. PRIME reports only conclusions authorized by its rules and ledger. With correct requirements, exact checks at known locations, and sufficient budget at stopping, completion reaches the strongest supported conclusion. On 480 public-record tasks, an agent shown the requirements reported unjustified conclusions on 26.7% of tasks, while PRIME reported none. Its directions and added checks raised the average score for justified conclusions from 30.1, with refusal alone, to the maximum of 59.2 out of 100.

==> sections/07_related.tex <==
\section{Related Work}
\label{sec:related}

Agents that interleave reasoning with tool calls \citep{yao2023react} have been made more reliable from the answer backwards: by self-critique and revision \citep{shinn2023reflexion,dhuliawala2023cove}, by checking statements against retrieved evidence \citep{chern2023factool,wei2024safe}, by withholding low-confidence claims with guarantees on the error rate \citep{mohri2024conformal,geifman2017selective}, and by gathering more evidence when a calibrated probability is uncertain \citep{zhang2026glean} or finding the smallest evidence set that verifies a draft \citep{li2024meg}; none fixes in advance which checks a conclusion requires or prevents the conclusion from being stated without them. Studies of agents that state a rule and then fail to act on it \citep{schmied2025greedy,reddy2026reasonless} and benchmarks of policy-following tool agents \citep{yao2024taubench} document the failure Experiment~A measures. The closest work enforces constraints from outside the model, shielding and rule enforcement on an agent's actions \citep{alshiekh2018shielding,wang2026agentspec,doshi2026safe} and control planes that admit a claim only on attested evidence under a contract fixed in advance \citep{researchloop2026,prooforstop2026,egvar2026}; PRIME shares their premise and differs in what it gates and feeds back: the conclusion, graded on a strength order, and the open requirements of the strongest reachable conclusion returned to the agent as its next work. Its ingredients are classical: minimal sufficient routes are prime implicants \citep{quine1952}, the object behind consistency-based diagnosis, truth maintenance, and abductive explanations \citep{reiter1987,dekleer1986atms,shih2018symbolic,ignatiev2019abduction}; the four-valued ledger descends from truth-maintenance systems; and how many costly tests to run before deciding is the question of sequential testing and active feature-value acquisition \citep{unluyurt2004sequential,deshpande2016approximation,saartsechansky2009active}. PRIME claims none of these; it adds their combination with a rule committed from the specification view, residual requirements that select the next admissible action, and an evaluation that scores each layer separately (Appendix~\ref{app:related}).


==> tab_multidoc.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrrrr}
\toprule
Method & \makecell[r]{Unsupported \%\\{}[95\% CI]} & Utility & \makecell[r]{Coverage\\\%} & \makecell[r]{Resolver\\error \%} & \makecell[r]{Quote\\precision \%} & \makecell[r]{Evidence\\read \%} \\
\midrule
\multicolumn{7}{l}{\emph{Not enforced}} \\
\quad Plain agent & 13.3 [9.0, 19.4] & 29.7 & 86.1 & -- & -- & 43.1 \\
\quad Fully informed agent & 12.1 [8.0, 18.0] & 38.2 & 91.5 & 44.4 & 77.9 & 38.3 \\
\quad RAG, as stated & 23.6 [17.8, 30.7] & 38.4 & 86.7 & 46.9 & 74.7 & 100.0 \\
\multicolumn{7}{l}{\emph{Enforced by the committed program}} \\
\quad PRIME & 12.1 [8.0, 18.0] & 36.0 & 82.4 & 52.9 & 73.1 & 49.4 \\
\quad PRIME, completion & 17.0 [12.0, 23.4] & 46.7 & 92.7 & 47.0 & 81.9 & 80.2 \\
\quad PRIME, verified & 6.1 [3.3, 10.8] & 27.5 & 60.6 & 37.8 & 78.2 & 47.9 \\
\quad PRIME, verified, completion & 9.7 [6.1, 15.2] & 45.5 & 86.1 & 37.3 & 83.1 & 84.4 \\
\quad Ceiling-targeting, model as resolver & 14.5 [10.0, 20.7] & 45.7 & 90.9 & 43.0 & 83.3 & 80.8 \\
\quad Ceiling-targeting, verified & 7.9 [4.7, 13.0] & 44.2 & 84.2 & 38.3 & 85.4 & 83.2 \\
\quad RAG, evidence-gated & 24.8 [18.9, 32.0] & 41.2 & 89.1 & 46.9 & 74.7 & 100.0 \\
\multicolumn{7}{l}{\emph{Ceiling-targeting with another resolver model}} \\
\quad gpt-oss-20b & 10.9 [7.0, 16.6] & 45.3 & 86.7 & 37.5 & 83.7 & 79.6 \\
\quad gpt-oss-20b, verified & 11.5 [7.5, 17.3] & 44.6 & 85.5 & 35.4 & 83.5 & 80.5 \\
\quad Mistral-Small-24B & 13.9 [9.5, 20.0] & 44.8 & 89.1 & 47.4 & 76.0 & 81.1 \\
\quad Mistral-Small-24B, verified & 7.3 [4.2, 12.3] & 37.8 & 72.7 & 36.9 & 80.7 & 86.8 \\
\bottomrule
\end{tabular}
\caption{Multi-document review on SciFact-Open: 165 claims, each with a packet of 2 to 8 expert-annotated abstracts (gold utility 54.3). Ceiling-targeting: the runtime picks each abstract the committed program's guidance selects and asks the model to judge it; no agent chooses an action. Completion: the runtime finishes PRIME's open obligations with that same judgment call, replayed from PRIME's logged stopping points. Verified: the blind verifier of Experiment~D admits a judgment only when a fresh-context second judgment agrees. Resolver error: accepted judgments that differ from the expert label; quote precision: accepted quotes on evidence abstracts that overlap an annotated rationale sentence; evidence read: annotated evidence abstracts the method read; -- marks fewer than 10 accepted judgments. Qwen2.5-32B-Instruct unless stated, greedy, 20 calls; the matched set is 165 of 165 claims.}
\label{app:tab:multidoc}
\end{table*}

